Repetition Neurons: How Do Language Models Produce Repetitions?

This paper introduces repetition neurons, regarded as skill neurons responsible for the repetition problem in text generation tasks. These neurons are progressively activated more strongly as repetition continues, indicating that they perceive repetition as a task to copy the previous context repeatedly, similar to in-context learning. We identify these repetition neurons by comparing activation values before and after the onset of repetition in texts generated by recent pre-trained language models. We analyze the repetition neurons in three English and one Japanese pre-trained language models and observe similar patterns across them.

==> latex/tables/invokingResults.tex <==
\begin{table}[]
\centering
\small
\begin{tabular}{lrr}
\hline
              & Random & Repetition \\ \hline
Gemma 2.8B    & 21     & \textbf{50}                \\
Pythia 2.8B   & 22     & \textbf{52}                \\
LLaMA 3.2 3B  & 45     & \textbf{69}                \\
LLM-jp-3 1.8B & 18     & \textbf{51}         \\ \hline
\end{tabular}
\caption{
    Number of samples in which the intervention to random and repetition neurons causes the repetition over 100 samples.
}
\label{tab:invokingRepetition}
\end{table}
